Reconstruct, Practice, Go Real: Guided Self-Improvement for Embodied Agents

Building reliable robot capabilities across diverse tasks requires substantial human effort to develop and maintain skills, design rewards, and integrate perception with control. We present Reconstruct, Practice, Go Real (RPG), a framework for autonomous improvement of robot execution systems without updating model weights. RPG identifies manipulation capabilities in an offline dataset and constructs related practice tasks in simulation. During practice, RPG uses execution feedback, privileged simulator state, and available dataset videos to diagnose failures. It develops new reusable symbolic skills, refines existing skills, and revises the system prompt based on these diagnoses. Cross-task evaluation tests individual candidate changes and merged revisions before they are retained for reuse. At test time, a multimodal LLM uses the resulting system prompt and skill library to coordinate perception and robot control. On held-out initializations of 22 manipulation tasks, RPG improves task success from 28.6% after the first practice round to 95.0% after 15 rounds, outperforming all evaluated baselines, including ASPIRE (75.5%) and CaP-Agent0 powered by GPT-6 Astra Pro (60.0%). After a common calibration and hardware-adaptation procedure, the frozen system succeeds in all 30 physical trials, with ten trials on each of three tasks. Project Website: https://rpg-robot.github.io/

==> tables/per_task_current.tex <==
\multicolumn{7}{@{}l}{\textbf{CaP-X tasks}} & \\
Lift cube & 9/10 & \textbf{10/10} & \textbf{10/10} & \textbf{10/10} & \textbf{10/10} & \textbf{10/10} & \textbf{10/10} \\
Nut assembly & 4/10 & 6/10 & 4/10 & 5/10 & 0/10 & 3/10 & \textbf{9/10} \\
Restack cubes & 6/10 & 9/10 & 8/10 & 7/10 & 5/10 & \textbf{10/10} & \textbf{10/10} \\
Spill wipe & 2/10 & \textbf{10/10} & 6/10 & 9/10 & 5/10 & 8/10 & \textbf{10/10} \\
Stack cubes & 8/10 & \textbf{10/10} & 9/10 & 7/10 & \textbf{10/10} & \textbf{10/10} & \textbf{10/10} \\
Two-arm handover & 5/10 & 3/10 & 3/10 & 6/10 & 2/10 & 6/10 & \textbf{10/10} \\
Two-arm lift & 2/10 & 3/10 & 3/10 & 2/10 & 6/10 & 8/10 & \textbf{10/10} \\
\textit{Group mean (\%)} & 51.4 & 72.9 & 61.4 & 65.7 & 54.3 & 78.6 & \textbf{98.6} \\
\midrule

\multicolumn{7}{@{}l}{\textbf{ABC-derived and analogous tasks}} & \\
Extract from fixture & 8/10 & \textbf{10/10} & 2/10 & 2/10 & 2/10 & 7/10 & \textbf{10/10} \\
Insert into fixture & 2/10 & 1/10 & 0/10 & 0/10 & 4/10 & 2/10 & \textbf{10/10} \\
Place dish on rack & 1/10 & 9/10 & 2/10 & 5/10 & 4/10 & 7/10 & \textbf{10/10} \\
Serve onto plate & 9/10 & \textbf{10/10} & 9/10 & 8/10 & 2/10 & \textbf{10/10} & 9/10 \\
Fold towel & 1/10 & 0/10 & 0/10 & 0/10 & 0/10 & 0/10 & \textbf{3/10} \\
Transfer object & 0/10 & 0/10 & 0/10 & 5/10 & 1/10 & \textbf{9/10} & \textbf{9/10} \\
Lift rod & 8/10 & \textbf{10/10} & 9/10 & \textbf{10/10} & \textbf{10/10} & \textbf{10/10} & \textbf{10/10} \\
Pick up cup & \textbf{10/10} & \textbf{10/10} & \textbf{10/10} & \textbf{10/10} & \textbf{10/10} & \textbf{10/10} & \textbf{10/10} \\
Place bottles in bin & 0/10 & 1/10 & 0/10 & 0/10 & 0/10 & 3/10 & \textbf{10/10} \\
Close sunglasses case & 9/10 & 6/10 & 6/10 & 6/10 & 9/10 & \textbf{10/10} & \textbf{10/10} \\
Close drawer & 6/10 & 5/10 & 6/10 & 3/10 & 9/10 & \textbf{10/10} & \textbf{10/10} \\
Sort cubes (standard)  & 3/10 & 2/10 & 4/10 & 5/10 & 1/10 & \textbf{10/10} & 9/10 \\
Sort cubes (extended) & 0/10 & 0/10 & 0/10 & 0/10 & 0/10 & 8/10 & \textbf{10/10} \\
Stack blocks & 4/10 & 7/10 & 0/10 & 1/10 & 2/10 & 5/10 & \textbf{10/10} \\
Transport cup & \textbf{10/10} & \textbf{10/10} & 9/10 & 7/10 & 0/10 & \textbf{10/10} & \textbf{10/10} \\
\textit{Group mean (\%)} & 47.3 & 54.0 & 38.0 & 41.3 & 36.0 & 74.0 & \textbf{93.3} \\
\midrule

\textbf{Mean success (\%)} & 48.6 & 60.0 & 45.5 & 49.1 & 41.8 & 75.5 & \textbf{95.0} \\
Total successes & 107/220 & 132/220 & 100/220 & 108/220 & 92/220 & 166/220 & 209/220 \\
